Sweeping Permutation Automata

This paper introduces sweeping permutation automata, which move over an input string in alternating left-to-right and right-to-left sweeps and have a bijective transition function. It is proved that these automata recognize the same family of languages as the classical one-way permutation automata (Thierrin, "Permutation automata", Mathematical Systems Theory, 1968). An n-state two-way permutation automaton is transformed to a one-way permutation automaton with F(n)=\max_(k+l=n, m <= l) k (l \choose m) (k - 1 \choose l - m) (l - m)! states. This number of states is proved to be necessary in the worst case, and its growth rate is estimated as F(n) = n^(n/2 - (1 + \ln 2)/2 \cdot n/(\ln n) \cdot (1 + o(1))).

==> eptcsdata.tex <==
\providecommand{\firstpage}{110}
\providecommand{\publicationstatus}{Rudolf Freund, Benedek Nagy (Eds.): 13th International Workshop on \\ Non-Classical Models of Automata and Applications (NCMA 2023)\\
EPTCS 388, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.388.11}{10.4204/EPTCS.388.11}}
\pdfoutput=1

